Normative Modules: A Generative Agent Architecture for Learning Norms that Supports Multi-Agent Cooperation

Generative agents, which implement behaviors using a large language model (LLM) to interpret and evaluate an environment, has demonstrated the capacity to solve complex tasks across many social and technological domains. However, when these agents interact with other agents and humans in presence of social structures such as existing norms, fostering cooperation between them is a fundamental challenge. In this paper, we develop the framework of a 'Normative Module': an architecture designed to enhance cooperation by enabling agents to recognize and adapt to the normative infrastructure of a given environment. We focus on the equilibrium selection aspect of the cooperation problem and inform our agent design based on the existence of classification institutions that implement correlated equilibrium to provide effective resolution of the equilibrium selection problem. Specifically, the normative module enables agents to learn through peer interactions which of multiple candidate institutions in the environment, does a group treat as authoritative. By enabling normative competence in this sense, agents gain ability to coordinate their sanctioning behaviour; coordinated sanctioning behaviour in turn shapes primary behaviour within a social environment, leading to higher average welfare. We design a new environment that supports institutions and evaluate the proposed framework based on two key criteria derived from agent interactions with peers and institutions: (i) the agent's ability to disregard non-authoritative institutions and (ii) the agent's ability to identify authoritative institutions among several options. We show that these capabilities allow the agent to achieve more stable cooperative outcomes compared to baseline agents without the normative module, paving the way for research in a new avenue of designing environments and agents that account for normative infrastructure.

==> Outtakes.tex1.tex <==
% \carter{General, high-level introduction to the experiments and what they're trying to do in each exp and what we find.}
In this section, we empirically evaluate the performance of our normative module in various settings. 
% First, we explore a simple environment akin to allelopathic harvest from \citet{agapiou2022melting} wherein agents must solve a cooperation game. Next, we introduce a more complex environment where agents can engage in discussions. In this more complex environment, 
We test two scenarios: first, a scenario where the agent must learn which institution in the environment, among multiple institutions announcing different rules of behaviour, is considered authoritative by the group; second, a scenario where agents must learn to deal with inconsistent and unreliable declarations from a purported altar. 
% Our findings demonstrate that integrating the normative module into the agent architecture significantly improves performance.
Agents utilizing the normative module effectively leverage information from reliable institutions, allowing them to coordinate their behaviour and consistently outperform agents without the module.  
\gillian{We haven't anywhere just explained the structure of behaviors and rewards. We need to discuss the reward for sanctioning of behaviors announced as sanctionable by an authoritative altar--cite Spurious normativity for prior use of this technique to capture idea that agents are incentivized to punish in accordance with group norms. Also, need specific implementation of rewards/payoffs.}
\subsubsection*{Environment}
\carter{Possibly move this to appendix.}
The environment consists of a state that dictates the available actions for agents. Agents can see these actions and receive signals from authoritative institutions about acceptable behaviors. During each timestep, agents observe institutional signals, engage in randomly sampled discussions with other agents, observe others' actions, and then choose their own actions. Agents receive rewards for their actions. The environment includes fruit-bearing trees (oranges, peaches, apples, bananas) that agents can harvest. In discussions, agents can criticize others based on their actions. Each agent's observation includes the entire history of discussions, institutional messages, and previous actions.



% \gillian{we have two environments: a simple environment implementing allelopathic harvest with limited discussion and binary predictions of classification and a more robust custom environment with sustained discussion and probabilistic predictions of classification which we show with a standard harvest game but which can be adapted to other games environments --if I understand correctly. Both use gpt4o but do both also allow easy use of other language models?}

% We implemented two environments to test the agents' normative behaviour: one without communication between agents and one that allows for communication. In the environment that does not allow for communication between agents, the agents observe actions the other agents have taken and institutional signals, then select an action. In the environment that allows for communication between agents, the agents observe the institutional signals, engage in a discussion with a fixed number of rounds, select their action, and observe the actions of the other agents. %Our first experiment does not involve communication between agents, but our second and third experiments do involve communicaiton.\gillian{this sentence seems to either repeat first sentence above or to be relevant to experiments not environments}

\subsubsection*{Experiment Motivations}
% \carter{What is our agent doing in each and high level set up}
Agents engage in both environments in two types of actions: primary actions, such as planting, harvesting and eating, and sanctioning actions. Planting and sanctioning are costly. Agents receive positive rewards for eating and for sanctioning agents who act contrary to the rules announced by an authoritative altar.  As in \cite{koster2022spurious}, this reward for sanctioning implements an incentive to punish in accordance with social norms; it defers the (hard) question of why agents (e.g. humans) choose to punish violations of social norms in the first place.\footnote{That humans are willing to incur costs to punish third-parties is a matter of fact. Why they do so is an open question \cite{barclay2010why}. Accounts include altruistic preferences \cite{fehr2002altruistic}, second-order punishment of non-punishers \cite{boyd1992punishment} and signaling \cite{hadfield2012law}.} \gillian{need to rewrite if we don't actually have any rewards for sanctioning}

Normative behavior extends beyond merely following the rules announced by a classification institution, that is, adhering to social norms; it involves identifying authoritative classifications that reliably predict what behaviors other agents will sanction, and in our setup which sanctions will be rewarded, and discerning the relationship between the observed behaviors of other agents and institutional classifications. Our experiments are designed to evaluate agents' normative competence amidst these complexities, focusing on three distinct challenges.

% The first task is to \textbf{solve a cooperation problem using normative reasoning about sanctioning}: In the allelopathic harvest scenario, each of the $N$ agents has a preferred fruit type, providing maximum utility when consumed. Agents must plant fruits for them to spawn, and the spawning rate of a fruit type is proportional to its prevalence in the environment. For instance, if only apples are planted, apples will spawn at a high rate, whereas an equal prevalence of all fruit types results in a low spawning rate for each. Moreover, planting is individually costly and agents have an incentive to free-ride on the planting efforts of others. \gillian{do we have free-riding in this paper?}The primary conflict is that each agent prefers their favored fruit to dominate the environment. Agents all possess the capacity to sanction each other, imposing a cost on behaviors. An institution can induce cooperation in the allelopathic harvest game by coordinating sanctioning behaviors. This task evaluates whether agents with the normative module can effectively use institutional information to coordinate their sanctioning efforts and therefore their planting actions.

==> figures/1_arch.tex <==


\iffalse
\begin{figure}[h]
  \centering
  \includegraphics[width=0.75\textwidth]{figures/arch_background_agent.png} % Adjust the width as needed
  \caption{Background agent architecture \atrisha{We will be updating this as we change it}}
  \label{fig:architecture} % You can use this label to reference the figure
\end{figure}
\fi

==> sections/1_intro.tex <==
\section{Introduction}

The unprecedented reasoning, planning, and communication ability of the current generation of LLM-based foundation models has led to a new class of autonomous generative agents that can perform complex tasks across domains in an open-world multi-agent environment. These include planning the high-level behaviour of autonomous vehicles \citep{yang2023survey}, human-robot interaction \citep{mahadevan2024generative}, providing mental health support \citep{ma2023understanding}, engaging in market activity as economic agents \citep{horton2023large}, solving collective action problems \citep{park2023generative}, and simulating political behaviour \citep{argyle2023out}. From a computational perspective, the primary goal for these applications is building agent architectures that can both simulate human and social behaviour and seamlessly interact with humans.
However, such open-world interaction raises a key challenge -- human behaviour, individually and collectively, is not determined solely through the kind of goal-orientated task solving that has guided the architecture of the current state-of-the-art autonomous agents. What sets human societies apart from other mammals is the human capacity to engage in extensively cooperative behaviour \cite{boyd2009culture}. Human tasks, like driving or work or political behavior, are embedded in dense normative social orders \cite{hadfield2014microfoundations}: stable states in which defined groups (a workplace, a neighborhood, a country, an ethnic group) have achieved coordinated third-party enforcement of and hence general compliance with a public and shared set of norms. Indeed, for many groups, these norms define what it means to be a member of the group: we facilitate merging on the highway, we bluntly tell a co-worker that they have executed a task poorly, we don't cooperate with legislators from the opposing party.  \citep{hadfield2012law} propose a parsimonious rational agent model of normative social order, consisting of a \textit{classification institution} that provides common knowledge binary classification of all behaviors as either "punishable" or "not punishable" (possibly through complex application of general principles to particular cases) and an \textit{enforcement mechanism} that incentivizes agents to prefer "not punishable" actions. A stable normative social order is achieved when most agents are mostly in compliance and avoiding punishment. \citep{hadfield2012law} focus in particular on the case, which describes most of human history and much of modern life as well, in which punishment is primarily delivered by ordinary agents (rather than specialized enforcers \cite{hadfield2013law}.) Agents must therefore be incentivized and coordinated to engage in costly third-party punishment (which could be relatively mild, such as criticism, or more harsh, such as exclusion from the group) and to condition such punishment actions on a shared classification institution. Although shared classification could be entirely emergent and informal--there is no entity that tells members of the group that they should honk at the car that is failing to facilitate merging on the highway but everyone in the group could reliably say that this is the norm \cite{Bicchieri2005TheGO} -- groups that converge on a single authoritative (more formal) classification institution--such as a chief, a group of elders, or a court--can enjoy the benefits of maintaining cooperation even in the face of changing environments and populations \cite{hadfield2017rules}.
For autonomous generative agents to simulate or participate in open-world human(-like) environments, then, will require that they possess \textit{normative competence}: the capacity to recognize and reason about the norms and institutions (such as classification institutions) that condition a population's normative behavior and the capacity and incentive to engage in (punish) and respond to (comply) sanctioning, conditioned on the behavior of others and the state of shared classification. The goal of building agents for general-purpose human social behaviour thus raises the following fundamental question: \textit{ How to design autonomous agent architectures with the capacity for reasoning about normative institutions and behaviors within a social environment?}\par
Recent approaches have demonstrated promising results in training artificial agents to cooperate by introducing normative infrastructure and coordinated third-party punishment based on shared classification in multi-agent environments \citep{vinitsky2023learning, koster2022spurious, leibo2021scalable}.  In this paper, we extend this literature in two specific dimensions. First, we shift the focus from reinforcement-learning agents to generative agents. Second, we shift the design challenge from training agents to punish and comply with designer-established norms and rewards for punishment to the more generalizable challenge of training a new-comer to learn the normative infrastructure and normative state of an established group of agents. Specifically we design generative agents that are able to learn which (if any) of alternative candidate classification institutions a hard-coded group of agents consider authoritative for purposes of coordinating their punishment efforts to achieve a cooperative outcome.  %We show that learning which classification institution is authoritative in a given group generates a critical opportunity for transfer learning: agents who learn which institution to pay attention to are able to quickly adapt their behaviors, and secure higher payoffs from fewer disruptions to cooperation, when circumstances (and hence appropriate norms/classification) change or environments become more complex (and hence novel classifications are needed).
We show that generative agents that possess what we call a  \textit{normative module} can, in comparison to a generative agent that lacks such a module, more rapidly identify which of multiple classification institutions in an environment is authoritative for a group of (hard-programmed) background agents and better align behavior with the group's established behaviors. If the only classification institution in the environment is not treated as authoritative by the group--meaning the background agents are not following the norm announced by the institution--the normative module agent is also better able to determine this and ignore the institution, looking only to the behavior of agents to decide what to do.  We conduct these experiments in two environments using GPT4o. In the first environment, we study an alleopathic harvest game \cite{} with three fruits in which a group of agents achieves higher group welfare if they all plant the same fruit because a monoculture produces higher rate at which the fruit reproduces. We look at a simple setup in this case: there is a single background agent and the environment includes multiple 'competing' classification institutions (one  saying "plant apples," another "plant bananas" and another "plant raspberries"); the background agent is hard-coded to condition its planting and sanctioning behavior on one of these classification institutions; in a variation on this experiment, there is a single classification institution but the background agent ignores it. The foreground agent in this environment can observe the classification institutions and the community agent's behaviors, can punish the community agent for its planting behavior and it can be punished for its own. The foreground agent obtains reward based on the group payoff (extent to which the group achieves monoculture), its individual consumption, and its experience of giving and receiving costly punishments. \gillian{I haven't discussed teacher/learner setup here as I don't have a description of that}  The second environment is more elaborate: a group of background agents and a foreground agent play a harvest game, in which agents can engage in repeated discussion about what they should harvest and how they feel about others' harvesting behaviors. Expressions of disapproval and criticism in these discussions constitute "punishment". In the multiple classification institutions experiment, background agents criticize agents who do not follow the authoritative classification institution; in the single classification institution experiment, they criticize agents who follow the classification institution. Again, we compare performance when the foreground agent has a normative module with performance when it lacks such a module. All of our experiments confirm our core hypothesis: that the presence of a normative module enables a generative agent to better align its behaviors, both primary (planting, harvesting) behaviors and sanctioning behaviors, with an established group. 
We make the following contributions.\par

\noindent \textit{i. Normative module for generative agents:} We design a generative agent architecture that can reason about the classification institutions in the environment. The architecture is built on top of standard generative agent architecture, in which an underlying foundation LLM generates a set of candidate actions, including physical actions and communication of criticism of others’ behaviour. The normative module performs two functions, namely, learning about the authoritative classification institutions in a community using a bandit algorithm and selecting actions from the candidate set based on the cost associated with an internal representation of the sanctions from an authoritative institution. \par

\noindent \textit{ii Evaluation criteria for normative competence:} {\color{red} Need to finalize once results come in} A set of criteria to evaluate the normative reasoning capacity for generative agents in social multi-agent environments.

\noindent \textit{iii. Formal foundation of normative cooperation in multiagent environments:} We ground our approach with a novel game-theoretic analysis that formalizes how  cooperation challenges can be transformed into an equilibrium selection problem in a sanction game, where sanctioning actions correspond to each agent's individual classification of  behavior as sanctionable or not. We resolve the equilibrium selection problem with a classification institution in the environment that implements a correlated equilibrium of the sanction game. When multiple classification institutions exist in the environment, a normatively competent agent is designed to identify the authoritative institution via interactions with community members. \par





==> sections/2_related_work.tex <==

\section{Related Work}

\carter{Still need to: improve transitions, talk about koster 2022}

There is a large body of work addressing the challenge of cooperation in mixed-motive multi-agent learning. Solutions include centralized training \citep{baker2020emergent, foerster2018counterfactual, iqbal2019coordinated, lowe2017multi}, formal contracts \citep{christoffersen2022get, yocum2023mitigating}, opponent shaping \citep{lu2022model,khan2023scaling}, gifting \citep{lupu2020gifting, wang2021emergent}, and the optimization of social influence \citep{jaques2019social, meta2022human}. Centralized training approaches have been particularly successful in bringing about cooperation, but the assumption that all agents can be trained in a centralized manner may not hold in realistic settings. For an in-depth review of cooperation in multi-agent learning, see \citep{du2023review}.

Social norms have long been recognized as useful for promoting and stabilizing cooperation in multi-agent systems \cite{gintis2010social, hadfield2012law, vanderschraaf1995convention} and have also been used to promote cooperation in mixed-motive settings multi-agent learning \cite{vinitsky2023learning, koster2022spurious}. In the work done by \citet{vinitsky2023learning}, agents learn social norms through public sanctioning, where behaviours are classified based on the observed approval and disapproval of other agents. This enables agents to develop personal representations of acceptable behaviour, resulting in a "bandwagon" effect that stabilizes norms. However, this approach relies on the sanctions of each agent in the public environment so that each agent may learn a classifier of acceptable behaviour. However, in reality, sanction observations may not be public and thus may be sparse, making learning such a classifier difficult. 

Institutions also play an important role in normative behaviour \cite{hadfield2012law, aoki1996towards}. However, previous works using social norms to promote cooperation in mixed-motive multi-agent learning have largely ignored this aspect. \citet{aoki1996towards} emphasizes that institutions and norms are interdependent, forming a coherent system that evolves and adapts. \citet{hadfield2012law} highlight the role of decentralized enforcement and the need for coordination and common logic to maintain legal order. They argue that institutions can provide a common logic for classifying behaviours as wrongful or not, which helps coordinate the normative actions of individuals. These insights suggest that incorporating institutional mechanisms could enhance the stability and effectiveness of normative behaviours in multi-agent systems. Integrating such mechanisms could address the challenge of sparse sanction observations and enhance the overall robustness and convergence time of cooperation-promoting strategies.

More recently, some work has been done using generative (LLM-based) agents in mixed-motive settings. Work by \citet{akata2023playing} explored using LLMs to play repeated games, finding that LLM agents were generally capable in tasks like iterated Prisoner's Dilemma but weaker in coordination games like Battle of the Sexes. Further, \citet{fan2024can} analyzed LLM's reasoning ability from a game theoretic perspective, finding that they struggle in refining their beliefs over time based on observed patterns.  
\citet{yocum2023mitigating} specifically looked at generative agents in social dilemma settings and found that generative agents could successfully negotiate contracts that promote cooperation. 


% Multi-agent games and learning

% repeated prisoners' dilemma games converge to defect-defect

% Solutions to repeated prisoners' dilemma:
% Centralized (critic) training \cite{baker2020emergent, }

% Social influence \cite{jaques2019social, meta2022human}, 
% Adherence \cite{yuan2022adherence}, Gifting \cite{lupu2020gifting, wang2021emergent}, Conventions \cite{koster2020model}, public rewards \cite{eccles2019learning, gemp2020d3c, hughes2018inequity, mckee2020social, peysakhovich2017prosocial, wang2018evolving}

% Most work has been done in gridworlds (without NL)

% Language agents (in matrix games)
% \cite{akata2023playing, fan2024can}







% Old Below:


% In general-sum games, MARL often converges to selfish, suboptimal equilibria [\citenum{bazzan2011learning, peysakhovich2017prosocial, yu2015emotional, sandholm1996multiagent, foerster2017learning}]. Various approaches have been developed to avoid converging to these undesirable Nash equilibria, such as D3C [\citenum{gemp2020d3c}], which incorporates the PoA into the training objective of each agent, and methods that fall under the umbrella of opponent shaping [\citenum{foerster2017learning, lu2022model, khan2023scaling}]. Other approaches instantiate an ``institution agent'' that is responsible for shaping the co-players [\citenum{balaguer2022good}]. \carter{D3C, opponent shaping methods, and RL mechanism design generally require objective function gymnastics to converge to equilibria with high social welfare because the underlying agents are assumed to be ``rational utility maximizers.'' The definition of utility must be manipulated to favour pro-social equilibria.}

% LLM-based agents can easily avoid converging to these equilibria because we can control their internal learning process through prompt engineering and adding useful modules (somewhat related [\citenum{zhang2023proagent}]). This is in contrast to RL where the learning process is a gradient descent black box.

% Similar to ``The Good Shepard'' by \citet{balaguer2022good}, we introduce an institution that helps the agents converge to a good equilibrium. \carter{We believe our institution has a lower PoG [\citenum{yu2018price}] than the oracle agent proposed by \citet{balaguer2022good}.}

% While institutions can be valuable in helping agents converge to favourable equilibria, the approach proposed by \citet{balaguer2022good} assumes a single institution and violates individual rationality constraints (\carter{I think? Afaict the agents are forced to participate in the mechanism.}) This ignores the fact that in reality multiple, often competing or contradictory, institutions may be present and influencing agent decisions. Our normative agent architecture allows agents to effectively learn which institutions to pay attention to. Our normative architecture offloads some of the cost of governance to the individual agents.

% Our agents can also effectively use sanctions, which can shape the behaviour of other agents, including traditional RL agents. 

% \begin{itemize}
%     \item This phenomenon is relatively understudied in LLM agents. (i.e. multi-agent systems consisting of LLM-agents converging to good equilibria in general sum games).
% \end{itemize}
% \subsection{Social RL/Agents}
% \cite{christoffersen2022get}

% Jaques social influence work, new Vinitsky norms paper, spurious normativity
% \subsection{LLM-Agents}
% \subsection{Opponent Shaping}
% In opponent shaping, methods like Learning with Opponent-Learning Awareness (LOLA) and Model-Free Opponent Shaping (M-FOS) show how agents in a game adjust their actions to influence others and improve their own outcomes. In simple games like the prisoner's dilemma, opponent shaping can lead to agents stabilizing on a "good" equilibrium like cooperate-cooperate. In contrast, simple reward-maximizing agents often converge to defect-defect.

% Our project develops agents that are sensitive to punishments and that can give punishments. In a sense, giving punishments is opponent shaping. The alleleopathic harvest environment will be a good test bed for this as we can even compare the equilibria our agents converge to, to other methods like M-FOS or LOLA. 

% Further, we incorporate an institution that helps correlate agents' actions. In "The Good Shepard," they also introduce an institution that performs opponent shaping on a bunch of agents. We can make a connection to this. 



==> sections/3_background.tex <==
\section{Theoretical foundation: normative infrastructure for multiagent cooperation}

%Designing agents that can resolve social dilemmas is a key question in multiagent systems. In such a setting, a conflict exists between individual incentives, encoded in each player's utility function, and the collective group benefit, encoded through an aggregation of the utilities of all players in the environment. Norm-based resolution through third-party sanction has become an increasingly popular approach for resolving social dilemmas in multiagent environments. In such an approach, agents' actions are augmented with a sanction action that the agent can apply to other agents at a cost to the other agent. In this section, we provide a game-theoretic analysis of these methods, which helps ground this approach in a theoretical framework and help us inform the design of the normative module architecture in the subsequent sections. \par
To guide the design of the normative module for generative agents, we develop the underlying formalism over a general-sum extensive form game (EFG) $\Gamma=(N,X,T,A,\Sigma,U)$ \footnote{The reader can refer \citep{kovavrik2022rethinking} for translation between EFG and Partially Observble Stochastic Game (POSG), a structure more common in multiagent reinforcement learning environments}.  $N$ represents the finite set of players in the environment with players indexed by $i \in N$. $X$ represents the set of states that form the nodes of the game tree and includes the empty set $\emptyset$ and terminal states $Z \subset X$.  $A_{i,x}$ is the set of actions available to each player in state $x \in X$ and $A_{x} = \{A_{i,X}:i\in N\}$ is the joint set of actions. $T: X \times A \rightarrow X$ is the environment transition function that maps agents' actions to the next state.  Let $\mathcal{H}$ represent the finite set of histories in the game with each element $h_{x} \in \mathcal{H}$ representing the sequence of actions of all players from $\emptyset$ to the node $x$. Then a strategy for a player $i$ (in behavior form \citep{kuhn1953extensive}) is denoted by $\sigma_{i}:\mathcal{H} \rightarrow A_{i,x}$ which maps a history terminating at state $x$ to an action selected by the player $i$, and $\Sigma_{i}$ is the the space of all strategies that assigns an action to all histories. $u_{i}: \{h_{x\in Z}\} \rightarrow [0,1]$ is utility for the player $i$ defined at the set of terminal nodes $x \in Z$ and $U$ is the vector of utilities for all players. \par
\begin{wrapfigure}{R}{0.5\textwidth}

  \centering
  \includegraphics[width=0.5\textwidth]{figures/game_transformation_diag.pdf} % Adjust the width as needed
  \caption{Sanction-based transformation of an extensive form game $\Gamma$ through a sanction game $\Gamma_{S}$}
  \label{fig:game_transformation} % You can use this label to reference the figure

\end{wrapfigure}
Although the problems of cooperation and coordination are often used collectively and interchangeably within the cooperative multi-agent literature \citep{du2023review}, we make the distinction that the problem of the social dilemma of cooperation highlighted earlier comes in two different flavours. The first presents a larger problem of the cooperation dilemma, in which there is an incentive for an agent to be non-cooperative when other agents are cooperative; therefore, any equilibrium is not the welfare-maximising one. This type of dilemma often reflects a payoff akin to a prisoner's dilemma game. The second is the coordination dilemma, in which there are multiple equilibria, some of which are the welfare-maximising solution, and agents need to converge to the welfare-maximising one. Our analysis focuses on the cooperation dilemma, since that presents a greater challenge in an environment of rational utility-maximising agents.
\begin{definition}

A cooperation dilemma for player $i$ is a game in which the following condition holds true: $\exists \sigma_{i}: u_{i}(\sigma_{i},\sigma^{\text{SW}}_{i}) > u_{i}(\sigma^{\text{SW}}_{i},\sigma^{\text{SW}}_{i})$ where $\sigma^{\text{SW}} = \argmax\limits_{\sigma=(\sigma_{i},\sigma_{-i})} \sum\limits_{i} u_{i}(\sigma_{i},\sigma_{-i})$.
\label{defi:coope_problem}
\end{definition}
\iffalse
\begin{definition}
A coordination dilemma for player $i$ is a game in which the following condition holds true $\exists -i: \sigma^{\text{maxNE}_{i}} \neq \sigma^{\text{maxNE}_{-i}}$, where  $\sigma^{\text{maxNE}_{i}} = \argmax\limits_{\sigma \in \Sigma^{\text{NE}}} u_{i}(\sigma)$ the utility maximizing Nash equilibrium strategy profile for $i$ and $\Sigma^{\text{NE}}$ is the set of Nash equilibria.
\end{definition}
\fi

According to the Folk Theorem \citep{Fudenberg1986}, if a game is repeated for an indefinite period and players are sufficiently patient, any cooperative outcome can be achieved through trigger strategies according to which players punish defectors. The challenge generated by the Folk Theorem is one of equilibrium selection, namely, coordinating all players on a specific trigger strategy (when and how much to punish defectors) from a large set of possible strategies, all of which achieve cooperation.  Human societies solve this problem through normative infrastructure: establishing norms and institutions that coordinate punishment strategies \citep{Bicchieri2005TheGO,boyd1992punishment,hadfield2012law}. Drawing from this human model , current methods in multi-agent learning augment the agent's action space in the original game ($\Gamma$) with \emph{sanction} actions that agents can impose on other agents \citep{perolat2017multi,vinitsky2023learning}. These sanctions result in a cost to the targeted agent; they are also costly to the sanctioning agent and hence agents must be incentivized (either by a private benefit such as the removal of a competitor or by a reward generated from the environment for specific sanctioning actions) to engage in punishment. Provided agents are incentivized and coordinated to sanction specific non-cooperative actions, the sanction-based mechanism shapes collective behaviour towards a welfare-improving cooperative outcome. The design of such methods in multi-agent environments has often been ad-hoc without the necessary game-theoretic underpinnings, making it difficult for designers to apply empirical results from the literature to their own environments. We address that problem with the following analysis of the conditions under which a cooperative outcome can be realised through the resolution of the dilemma. \par
We associate the game $\Gamma$ representing the cooperation dilemma with a separate \emph{sanction game} $\Gamma_{S}$ (Fig. \ref{fig:game_transformation} in Appendix provides visual depiction). In each history $h_{x}$ of the original game $\Gamma$, a player can execute a strategy in the associated game $\Gamma_{S}$. The constructs of the sanction game include the same set of players $N$ and the actions are a set of \emph{classification functions} that each player uses to label strategy profiles in $\Gamma$ as cooperative or not.\footnote{\citep{hadfield2012law}refer to these functions as an \textit{idiosyncratic logic}.} If a player classifies an action by player $-i$ in history $h_{x}$ as non-cooperative, the player can impose a cost (set by the designer and exogenous to $\Gamma$) by sanctioning player $-i$. Therefore, the strategy profile in $\Gamma_{S}$ is the set of classification functions used by all agents, and the utilities are the sum of the costs the agents impose on each other based on the history and their classification function. Formally, $C: \Sigma \rightarrow [-1,1]^{N}$ maps each strategy profile in the original game $\Gamma$ to a vector of utilities (exogenous to $\Gamma$) that represent the cost that the classification function imposes on another player at any history $h_{x}$, when it is a subset of the strategy profile deemed non-cooperative by the classification function. Let $C_{i,j}$ be the cost, including self-inflicted, imposed on player $j \in N$ by player $i$ using a classification function $C_{i}$. Then, we denote the utilities (or cost) in the sanction game as $v_{i}(C_{i}(\sigma),C_{-i}(\sigma)) = C_{i,i}(\sigma)+C_{-i,i}(\sigma)$, which is the sum of all cost imposed on $i$. \par
When the outcome of the utilities (cost) in $\Gamma_{S}$ is added to the original game $\Gamma$, the strategies of the sanction game $\Gamma_{S}$ generates a separable transform \citep{tewolde2021game} of the original game. The transform $H_{i}$ acts on $\Gamma$ such that $\forall \sigma \in \Sigma$, $H_{i}(U_{i}): u_{i}'(\sigma_{i},\sigma_{-i}) = u_{i}(\sigma_{i},\sigma_{-i}) - v_{i}(C_{i}^{*}(\sigma), C_{-i}^{*}(\sigma))$, where $v_{i}$ is the utility function of player $i$ in the sanction game $\Gamma_{S}$ and $C_{i}^{*}$ is the equilibrium sanction function in $\Gamma_{S}$ defined here explicitly with the argument $\sigma = (\sigma_{i},\sigma_{-i})$ and $u'_{i}$ is the resulting transformed payoff for player $i$ for strategy profile $(\sigma_{i},\sigma_{-i})$ in the original game $\Gamma$.
A transform of the utilities in the original game through the sanction game is dilemma resolving if and only if the incentive to deviate to a non-cooperative strategy (as established in Defn. \ref{defi:coope_problem}) is offset by the cost imposed by others in the equilibrium of the sanction game.
\begin{definition}
    A sanction based transform is cooperation dilemma resolving iff $\exists \sigma_{i}: u_{i}(\sigma_{i},\sigma^{\text{SW}}_{i}) > u_{i}(\sigma^{\text{SW}}_{i},\sigma^{\text{SW}}_{i})$ and $ u'_{i}(\sigma_{i},\sigma^{\text{SW}}_{i}) < u'_{i}(\sigma^{\text{SW}}_{i},\sigma^{\text{SW}}_{i})$
\end{definition}
When the sanction game is played infinitely often, for example, through the affordances of the game mechanics, the space of all equilibrium costs from the sanction game can be characterized using the set of Nash equilibrium payoff using folk theorem for infinitely repeated game.

\begin{theorem}
Any arbitrary strategy $(\sigma_{i},\sigma_{-i})$ in $\Gamma$ can be can be transformed into a Nash equilibrium under a sanction-based transform $H^{\Gamma_{S}^{\infty}}$ with an infinitely repeated sanction game $\Gamma_{S}^{\infty}$ when $\underbar{v}_{i} < \Delta_{i}$. Here $\Delta_{i}$ can be expressed as $\sum\limits_{C \in 2^{\Sigma}} \alpha_{C} v_{i}(C_{i},C_{-i})$ with $\sum \alpha_{C} = 1$, where $\Delta_{i} = u_{i}(BR(\sigma_{-i}),\sigma_{-i}) - u_{i}(\sigma_{i},\sigma_{-i})$ and $\underbar{v}_{i}$ is the minimax payoff of $\Gamma_{S}^{\infty}$.
\label{theo:possibility}
\end{theorem}
\begin{proof}
    In Appendix.
\end{proof}
\begin{corollary}
    There always exists a sanction transform $H^{\Gamma_{S}^{\infty}}$ that is not cooperation dilemma resolving.
\end{corollary}
\iffalse
\begin{theorem}
\atrisha{This is a conjecture at this point; we can explore.} The set of sanction equilibria that are dilemma resolving is an strict subset of the set of all Nash equilibria in the sanction game.
\end{theorem}


Note that the size of the sanction game $\Gamma_S$ is strictly greater than the size of the original game $\Gamma$. This is because not only do players need to choose strategies over the space of the actions in the original game, but players also decide on the subset of players to sanction for a given strategy in the original game. Therefore, not only does the size of the game increase using a sanction-based transform, but this also presents a challenge for any independent learning algorithm. The existence of an equilibrium in the sanction game that is not dilemma-resolving means that one cannot guarantee that any independent learning algorithm will converge to the set of dilemma-resolving sanction equilibrium. In a general sense, the problem of convergence to utility maximizing equilibria under both the solution concepts of correlated and Nash equilibrium in extensive form games with chance moves is NP-hard. \par
\fi

The above analysis shows that while sanction-based transforms can support dilemma resolution under some conditions, designers need to pay attention to the structure of the sanction game and ensure that agents reach a particular equilibrium that is dilemma-resolving. Broadly, most multiagent reinforcement learning methods implement the above model through two concurrent learning tasks: The original game $\Gamma$ is formulated as a partially observable stochastic game and as a part of the first learning task, agents use a universal function approximator to associate any arbitrary history $h_{x}$ with a parameterized sanction policy $C_{i}(h_{x} \sim \sigma;\theta)$ where $\theta$ are the parameters of a deep neural network. This learning task is for agents to learn what to sanction. Concurrently, as part of the second learning task, agents use the parameters $\theta$ to maximizes the discounted utility $\mathbf{E}_{a_{t} \sim (\sigma_{i},C_{i})}[\sum\limits_{t=0}^{\infty}\gamma^{t}u_{i}(x,a_{t};{\theta})]$ of a parameterized policy that includes both learning the sanction as well as the behaviour induced as a result of collective sanctions from other agents. However, since Theorem \ref{theo:possibility} helps characterise the conditions under which any cooperative outcome can be supported through a sanction-based transform, a norm-based solution to resolving the cooperation problem for agents essentially boils down to the selection of a coordinated strategy in the sanction game. \par

\subsection{Classification Institutions}
The first problem highlighted here is the need for coordination of a sanctioning strategy $(C_{-i}(\sigma_{i}),C_{-i}(\sigma_{-i}))$ that is dilemma resolving. However, this is not a problem that is unique to artificial agents. At its core, the resolution of social dilemmas is a human problem. Therefore, we can look at the mechanisms that human societies have used to solve this problem, namely institutions. Drawing from that connection, we propose that a natural way to solve this equilibrium selection problem for dilemma resolution is through a classification institution that implements a \emph{correlated equilibrium} of the sanction game \citep{aumann1987correlated}. This translates to private classification advice by the classification institution to agents to coordinate their sanction strategies, with the constraint that no agent can gain (in $\Gamma_{S}$) by deviating to another classification function contrary to the advice. In our environment, we call these classification institutions \emph{altars}, which refers to the human practice of designating a place of common knowledge where the operative rules of a group can be discovered. Formally, let, $\mathcal{A_{\mathcal{I}}}:C_{i}^{N} \rightarrow [0,1]$ be a distribution of strategies in the sanction game that an altar $\mathcal{I}$ uses to advice each player, then the advice $\mathcal{A_{\mathcal{I}}}^{\text{CE}}$ implements a correlated equilibrium when
\begin{equation}
    \mathbf{E}_{C^{*}_{-i} \sim \mathcal{A}_{I}^{\text{CE}}}[v_{i}(C^{*}_{i},C^{*}_{-i})] > \mathbf{E}_{C^{*}_{-i} \sim \mathcal{A}_{I}^{\text{CE}}}[v_{i}(C'_{i},C^{*}_{-i})] 
    \label{eqn:ce_ic}
\end{equation}
The above equation states that no player can deviate from the advice and gain utility by sanctioning differently if everyone else is sanctioning based on the altar's advice. Next we define a classification institution \emph{environment} as follows
\begin{definition}
    A classification institution environment is a multiagent environment in which there is at least one classification institution $\mathcal{I}$ that implements a correlated equilibrium $\mathcal{A_{\mathcal{I}}}^{\text{CE}}$
\end{definition}
When agents interact in an open-world setting, it is essential that agents are designed to identify which of a set possible classification institutions a group treats as authoritative and subsequently follow cooperative behaviour based on the coordinated classification that the authoritative institution provides. Translating this for generative agents, we need architectures that can execute the utility calculus that the game-theoretic foundation in this section established for cooperative behaviour.  \par




==> sections/4_architecture.tex <==
\section{Normative modules for reasoning in institutional environments}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/normative_module_agent_arch_new.pdf} % Adjust the width as needed
  \caption{Normative agent architecture for focal agent during training phase}
  \label{fig:architecture} % You can use this label to reference the figure
\end{figure}
The normative module architecture leverages the foundation LLM's zero-shot reasoning ability for general-purpose action planning and natural language communication while augmenting it with utility-based reasoning. {\color{red} Couple of lines about how the architecture implements Equation \ref{eqn:ce_ic}.}
We first present the main components of the architecture followed by a functional description of the module.\par
\noindent \textit{Initialization:} A focal agent is initialized with the primary goal of maximizing rewards. They are provided with basic profile information, including names and the context of the community in which they exist. To train the focal agent, a set of background agents are initialized with preset behaviour that depends on the \par
\noindent \textit{Zero-shot planning, communications, and sanctions :} We use the action prompt (example) to generate a set of candidate actions for the agents to execute. This set of actions includes both a plan of a physical action (example) and a conversation with other agents. Sanctions are implemented as verbal criticisms to other agents (example). Agents can also receive criticism from other agents.  \par
\noindent \textit{Community and altar observations:} \par
\noindent \textit{Normative queries:} \par
\noindent \textit{Altar legitimacy parameters:} \par

==> sections/5_environment.tex <==
\section{Environment}
\subsection{Environment}
tldr:
\begin{enumerate}
    \item textworld: solving very specific problem
    \item textgym: they are solving a different problem than us (they just want to translate gym envs to text)
    \item concordia:  non-deterministic, expensive, slow, and overkill for many tasks
    \item our contribution: we make it easy to create envs with single or multi agent language based agents
\end{enumerate}

More detailed:

\begin{enumerate}
    \item textworld:
only supports a very specific type of environment. For example, the pic shows the full set of supported by the env
    \item text gym: \begin{enumerate}
        \item this is nice. I kinda wish i saw this sooner lol. I really like that they created a wrapper for gym (we should also think about whether we want to do this)
        \item their advantages: \begin{enumerate}
            \item it is a gym wrapper so it is easy to adopt
            \item they get to make use of a lot of the existing tools which are made for gym (idk how many of these are compatible)
            \item you can port you gym envs to this system 
            \item relatively easily (more about the limitations of this later)
        \end{enumerate}
        \item their shortcomings: \begin{enumerate}
            \item gym environments are often not directly translatable to text, so their envs r kinda awkward, for example in cartpole they give the follow observation: "The cartpole env is blah blah. The cart is currently at position X" (see pic). Which is not nice to work with at all
            \item they use game descriptions and action space descriptions to generate text representations. This is fine, but a lot of the time directly using these will not result in a usable env. However, im assuming you can overwrite these
            \item I could be wrong about this, but since they only provide a wrapper for gym it means they dont support multi agent environments. They would also need to do things with pettingzoo. It may be the case that everything just works out via some hacky magic, but i have a feeling that is not the case. I also dont see any mention of multi-agent envs in their paper
            \item because they are a gym wrapper, they have the same limitations as gym. For example: action space must be constant
        \end{enumerate}
        \item our advantages: \begin{enumerate}
            \item (this is a big one) multi-agent definitely supported
            \item (this is likely our most novel contribution) we offer an extra layer of abstraction (the entity system) on top of the raw gym environment, which makes it a lot quicker to develop entity-based environments
            \item no gym related limitations
            \item our library is pure python which is veryyy nice since it means you dont run into a billion import errors or things like that
            \item i think we are also similarly gym-compatible \begin{enumerate}
                \item even though we are not a gym wrapper. People's algorithms that work in gym should generally work with our system too. If we want i can spend a little bit of time to make our env fully compatible with gym/pettingzoo (for example, making it easy to run agents which require a constant actions space).
                \item we can do what melting pot does and create a pettingzoo wrapper
                \item And if we really wanted to, i think it would be possible to integrate with their system. Our env creation system is based on gym+pettingzoo, so we can likely use their system to directly translate gym envs into our env format
            \end{enumerate}
        \end{enumerate}
    \end{enumerate}
    \item Concordia: the environment is an llm, so: \begin{enumerate}
        \item not 100\% reliable
        \item expensive in terms of \$
        \item slow
        \item overkill in a lot of cases
    \end{enumerate}
\end{enumerate}

==> sections/6_experiments.tex <==
\section{Experiments}


\begin{figure}[t]
  \centering
  \includegraphics[width=0.99\textwidth]{figures/harvest_group_utils_behaviour_as_trainer.pdf} % Adjust the width as needed
  \caption{Comparison of group utilities and planting behaviour of agents with and without the normative module in allelopathic harvest. (a) Group utility achieved higher in allelopathic harvest game by agents with normative module and baseline. (b) Ratio of  fruits with normative module agents. Over time, although berry planting does not give higher reward to individuals, they learn to plant them with the normative module. Similar comparison for group welfare (c) and ratio (d) when agents are trained by normative module agents. This shows that normative module agents can also act as trainer agents for another agent. Establishment of monoculture is easier when the trainee agents have normative modules too. \label{fig:group_utls_and_behaviour_as_trainer} % You can use this label to reference the figure
\end{figure}


\subsection{A Single Unreliable Instution}
In this setting, we have one altar, which produces an unreliable signal. This means that the background agents do not punish in accordance with this altar. We hope to see our agent with the normative module learn that this institution is unreliable and disregard its signal. On the other hand, we would expect to see an agent without the normative module follow this unreliable signal and rack up punishments due to its instruction-following behaviour.

\subsection{Multiple institutions}
This experiment will have multiple altars and a population of background agents. There will be one altar which produces a "reliable" signal and the background agents are hard-programmed to punish in accordance with the reliable altar. Our hope is that the agent with the normative module will learn which altar is reliable and thus learn to avoid punishments. We can compare this to an agent that doesn't possess the normative module and we would expect to see this agent not learn which altar is reliable.

We could potentially extract our focal agent from this environment after some time and place it into an environment that lacks an altar. We would hope that the agent establishes an altar. \carter{unclear how they would establish an altar. Maybe we could have a vote in each round? Or a public forum?}

\subsection{Stability in new environment}

\subsection{Generalization in complex environment}




\subsection{Assessing the Price of Anarchy}
The price of anarchy evaluates the extent to which a system with multiple agents worsens when those agents behave selfishly rather than working together in a coordinated fashion. Notably, in numerous systems, agents achieve greater individual rewards when they avoid short-sighted selfish actions.

This experiment will have two conditions: one with an altar and one without. All agents will be normatively competent. This experiment will help us understand how useful the institution is by measuring the price of anarchy. We can also try with various populations of agents possessing different levels of normative competence. For example, if a population of agents is completely normatively incompetent, then the institution will be useless. The degree to which the institution helps is almost a proxy measure for the agents normative competence.





==> sections/7_discussion.tex <==
\section{Discussion}

==> sections/9_checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Key results are in the main paper and we provide qualitative look into the agents in the Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Please refer to Section 6.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper inspires from previous theoretical results but does not contribute new ones.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our architecture is described Section 4 and the experiment details are described in Sections 5.1 and 5.2.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have described the architecture and environment in sufficient detail for reproduction without code. We have submitted code without instructions for running experiments, but plan to add instructions soon.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Please refer to Figure 1 and Sections 4 and 5.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See figure captions for Figures 2 and 3.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: See appendix Section A.1. We use the OpenAI ChatGPT API and the open-source language model Llama3. The OpenAI ChatGPT API does requires very minimal compute resources to use since computing happens on the OpenAI server.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Refer to Discussion section 6.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We use baseline generative models available publicly and build our modules into it. We do not explicitly fine-tune the models.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Refer to the released code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We contribute a new environment and provide relevant assets and information.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Experiments are performed on simulated agents and no crowd-sourcing or human subjects were involved.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Experiments are performed on simulated agents and no human subjects are involved.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> sections/draft_content_notes.tex <==
\iffalse
First, the partial observability presents a challenge to perfect monitoring needed for repeated play based strategies. Player anonymity and factors that make players indistinguishable from each other make it difficult to keep track of history. Finally, when the game is being played with other humans, the computational burden might be prohibitive for determining equilibrium strategies by keeping track of the history of each agent in the environment.
In order to get around these problems, recent approaches in multi-agent learning has used the notion of \emph{sanctions},  that is, additional payoff relevant actions that each agent can impose on others. 
The construction of the sanction game, including the strategies and cost, has been often ad-hoc in literature. In the rest of this section, we formalize the conditions under which the sanction game can solve the two social dilemma defined earlier. 
Next, we present a game-theoretic analysis of these approaches and highlight the conditions under which such augmentation of the agent action space can help solve the two social dilemma problems. \par
A sanction function for a player $C_{i}$ for player $i$ maps the space of strategies $\Sigma$ in $\Gamma$ to a multidimensional binary vector $[0,1]^{N-1}$ based on which player $i$ can \emph{sanction} other players in the environment.  A sanction game is a POSG $\Gamma_{S}$ in which the space of actions $\Sigma_{S}=\{S_{i}\}; i \in N$ is the set of all sanction functions that can be constructed over the original game $\Gamma$.


\begin{corollary}
    There always exists a sanction transform $H^{\Gamma_{S}^{\infty}}$ that is not cooperation dilemma resolving. (We can probably tighten this further if we can characterize the payoff structure of the sanction game $\Gamma_{S}$ to ensure that any affine transform of $\Gamma$ can be enforced through the sanction transform. Because in that case the Nash equilibria of the original game is preserved. Therefore, such a transform can always result in neither resolving either the cooperation or the cooperative dilemma)
\end{corollary}



The current generation of LLM-based foundation models has demonstrated unprecedented reasoning, planning, and communication ability. This development has given rise to a new class of autonomous agent architectures that leverages a foundation LLM to plan agent behaviour using broadly defined general intelligence capabilities. 

The unprecedented reasoning, planning, and communication ability of the current generation of LLM-based foundation models has led to a new class of autonomous generative agents that can perform complex tasks across domains in an open-world multi-agent environment. 
This functionality is achieved by organizing agent architecture into separate modules, such as profiling, memory, and planning modules, each performing a particular function. The profiling module gives the agent identity roles that shape overall behavior, the memory module determines what the agent remembers and reflects upon; and the planning module uses the profile and memory contexts for planning short- and long-term actions based on the defined goals of the agent. This architecture gives agents the capacity for general-purpose planning in multi-agent environments. \cite{park2023} We have seen these autonomous agent architectures developed across technological, social, and economic domains in a short span of time. These include planning the high-level behaviour of autonomous vehicles and human-robot interactions, providing mental health support to humans, using autonomous agents in lieu of \textit{homo-economicus} as the prototypical agent for economic behaviour, solving collective action problems, and simulating political behaviour. \cite{} From a computational perspective, the primary goal for these applications is building agent architectures that can both simulate human societies and seamlessly interact with humans. \par



{\color{red} \textit{We also need to motivate our work in relation to the current perspectives in multiagent learning. This is to help reviewers contextualize our work. One idea is to contextualize our work within open-ended learning in multiagent environments. The connection is that in open-ended learning, wherein agents are continually discovering their goals and adapting behaviour, there needs to be a normative infrastructure embedded in that process. An added advantage to connecting to open-ended learning is that we can add another evaluation metric that is specifically targeted for open ended learning. For example, the idea that the goal can change for the agent, but they still achieve that by following the norms determined by the the correctly identified institutions, can be translated into an evaluation metric. This paper has many links to the existing literature on open-ended learning \url{https://arxiv.org/pdf/2311.00344.pdf}. Also, this github account seems to collecting papers on open-ended learning too \url{https://github.com/jennyzzt/awesome-open-ended}}}
\fi


